Sonet Network Design Problems

This paper presents a new method and a constraint-based objective function to solve two problems related to the design of optical telecommunication networks, namely the Synchronous Optical Network Ring Assignment Problem (SRAP) and the Intra-ring Synchronous Optical Network Design Problem (IDP). These network topology problems can be represented as a graph partitioning with capacity constraints as shown in previous works. We present here a new objective function and a new local search algorithm to solve these problems. Experiments conducted in Comet allow us to compare our method to previous ones and show that we obtain better results.

==> algorithm2e/algorithm2e_ex01.tex <==
\SetVline
\eIf{cond1}{
  a line\;
  a line\;
}{
  another line\;
  another line\;
}


==> algorithm2e/algorithm2e_ex02.tex <==
\SetNoline
\If{cond2}{
  second if\;
  second if\;
}


==> algorithm2e/algorithm2e_ex03.tex <==
\lIf{cond3}{ another example}
\Else{
  a block\;
  a block\;
}


==> algorithm2e/algorithm2e_ex04.tex <==
\lIf{cond4}{ok} \lElse{wrong}\;

==> algorithm2e/algorithm2e_ex05.tex <==
\SetVline
\lIf{cond5}{cond5 true}\;
\uElseIf{cond51}{
  cond 5 false\;
  but cond51 true\;
}
\ElseIf{}{
  all is wrong\;
  \Return result52\;
}


==> algorithm2e/algorithm2e_ex06.tex <==
\SetLine
\uIf{cond6}{
  cond6 is ok\;
  always ok\;
}
\uElseIf{cond62}{
  choose result62\;
  \Return result62\;
}
\Else{
  all is wrong\;
  do something else\;
}


==> algorithm2e/algorithm2e_ex07.tex <==
Let's have a look at what we can do
with if-then-else and side comments\;
\eIf{if-then-else test}{
  no comment here\;
  neither in then\;
}{
  nor in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  then with a comment\;
}(\tcc*[f]{comment in else})
{
  here we are in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  again a comment in then\;
}{
  but not in else\;
}
\eIf{if-then-else test}{
  this time, no comment in then\;
}(\tcc*[f]{else comment})
{
  but one comment in else\;
}
Let's try with other if possibilities\;
\lIf(\tcc*[h]{lif comment}){test}{text}
\uIf(\tcc*[f]{uif comment}){test}{
  then text\;
}
\uElseIf(\tcc*[f]{comment}){test}{
  elseif text\;
}
\lElseIf(\tcc*[h]{comment}){test}{text}
\lElse(\tcc*[f]{comment}){text}


==> algorithm2e/algorithm2e_exfor.tex <==
\SetLine
\ForAll{elements of $S_1$}{
  remove an element e from $S_1$\;
  put e in the set $S_2$\;
  }
\lFor{i=1 \emph{\KwTo}max}{mark i}\;
\ForEach{$e$ in the set}{
  put $e$ in ${\cal E}$\;
  mark $e$\;
}


==> algorithm2e/algorithm2e_exrepeat.tex <==
\Repeat{this stop condition}{
  the text of the loop\;
  another line\;
  always in the loop\;
  }
\lRepeat{stop}{a one line loop}


==> algorithm2e/algorithm2e_exswitch.tex <==
\Switch{the value of T}{
  \uCase{a value}{
    do this\;
    do that\;
  }
  \lCase{another value}{one line}\;
  \Case{last value}{
    do this\;
    break\;
  }
  \Other{
    for the other values\;
    do that\;
  }
}

